On the structure of normalized models of circular-arc graphs -- Hsu's approach revisited

Circular-arc graphs are the intersection graphs of arcs of a circle. The main result of this work describes the structure of all \emph{normalized intersection models} of circular-arc graphs. Normalized models of a circular-arc graph reflect the neighborhood relation between its vertices and can be seen as its canonical representations; in particular, any intersection model can be made normalized by possibly extending some of its arcs. We~devise a data-structure, called \emph{PQM-tree}, that maintains the set of all normalized models of a circular-arc graph. We show that the PQM-tree of a circular-arc graph can be computed in linear time. Finally, basing on PQM-trees, we provide a linear-time algorithm for the canonization and the isomorphism problem for circular-arc graphs. We describe the structure of the normalized models of circular-arc graphs using an approach proposed by Hsu~[\emph{SIAM J. Comput. 24(3), 411--439, (1995)}]. In the aforementioned work, Hsu claimed the construction of decomposition trees representing the set of all normalized intersection models of circular-arc graphs and an $\mathcal{O}(nm)$ time isomorphism algorithm for this class of graphs. However, the counterexample given in~[\emph{Discrete Math. Theor. Comput. Sci., 15(1), 157--182, 2013}] shows that Hsu's isomorphism algorithm is incorrect. Also, in a companion paper we show that the decomposition trees proposed by Hsu are not constructed correctly; in particular, we showed that there are circular-arc graphs whose all normalized models do not follow the description given by Hsu.

==> data_structure_new.tex <==
\section{Conformal models of~$G_{ov}$}
\label{sec:data_structure}

Let $G = (V,E)$ be a circular-arc graph with no twins and no universal vertices,
$G_{ov}=(V,{\sim})$ be the overlap graph of~$G$, and let $\strongModules(G_{ov})$ 
be the modular decomposition tree of~$G_{ov}$.

\begin{definition}
Let $\phi$ be a conformal model of $G_{ov}=(V,{\sim})$ and let $M$ be a child of $V$ in $\strongModules(G_{ov})$.
A set $S \subseteq V$ is called a \emph{CA-module} of $M$ in the conformal model $\phi$ if $S$ is inclusion-wise maximal module of $G_{ov}$ such that the following two conditions hold: (i)~$S \subseteq M$ (ii)~$S$ induces a consistent permutation model in $\phi$.
\end{definition}
Given a conformal model $\phi$ of $G_{ov}$ and a child $M$ of $V$ in $\strongModules(G_{ov})$, 
we denote by $\camodules_{\phi}(M)$ the set of all CA-modules of $M$ in $\phi$.
The next lemma summarizes the properties of the sets $\camodules_{\phi}(M)$.
\begin{lemma}[\cite{Kra24}]
\label{lem:CA-modules}
Let $M$ be a child of $V$ in $\strongModules(G_{ov})$. 
Then:
\begin{enumerate}
\item \label{item:CA-modules-partition} For every conformal model $\phi$ of $G_{ov}$ the set $\camodules_{\phi}(M)$ forms a partition of the set $M$. 
\item \label{item:CA-modules-definition} For every two conformal models $\phi, \phi'$ of $G_{ov}$ we have $\camodules_{\phi}(M) = \camodules_{\phi'}(M)$.
\item \label{item:CA-modules-orientation} For every two conformal models $\phi, \phi'$ of $G_{ov}$, every $S \in \camodules_{\phi}(M)$, and every $x,y \in S$ the relative orientations of 
the chords representing the vertices $x$ and $y$ in the consistent permutation models induced by $S$ in the model $\phi$ and in the model $\phi'$ is the same (that is, in both those models the chords $\phi(x)$ and $\phi(y)$ either have the same or have different orientations).  
\end{enumerate}
\end{lemma}
For every child $M$ of $V$ in $G_{ov}$ let
$$\camodules(M) = \camodules_{\phi}(M),\quad \text{where $\phi$ is a conformal model $\phi$ of $G_{ov}$,}$$
and let
$$\camodules = \bigcup \big{\{}\camodules(M): M \text{ is a child of $V$ in $\strongModules(G_{ov})$} \big{\}}.$$
The members of the sets $\camodules(M)$ and $\camodules$
are called the \emph{CA-modules} of $M$ and of $G$, respectively.
Note that, by Lemma~\ref{lem:CA-modules}.\eqref{item:CA-modules-definition}, the sets $\camodules(M)$ and $\camodules$ do not depend on~$\phi$.
Note also that Lemma~\ref{lem:CA-modules}.\eqref{item:CA-modules-definition} asserts that each 
CA-module induces a consistent permutation model in any conformal model of $G_{ov}$.

Assume that $\camodules = \{S_1,\ldots,S_t\}$ is the set of all CA-modules of $G_{ov}$.
We pick a vertex $s_i$ in every set $S_i$, called the \emph{representant} of $S_i$.

Let $i \in [t]$. 
Lemma \ref{lem:CA-modules},\eqref{item:CA-modules-orientation} asserts there is a partition $\{S^0_i,S^1_i\}$ of the set $S^*_i$ such that for every conformal model $\phi$ both the sets $S^0_i$ and $S^1_i$ are contiguous in $\phi$ and
$(\phi|S^0_i, \phi|S^1_i)$ is a consistent permutation model induced by $S_i$ in $\phi$.
Note that $\{S^0_i, S^1_i\}$ is a partition of $S^*_i$ and $|\{s^0,s^1\} \cap S^0_i|=1$ and $|\{s^0,s^1\} \cap S^1_i|=1$ for every $s \in S$.
We assume the superscripts in $S^0_i,S^1_i$ are chosen such that $s_i$ is oriented from $S^0_i$ to $S^1_i$.
Since for every conformal model $\phi$ the relative orientation of the chords in $(\phi|S^0_i,\phi|S^1_i)$ is the same and since $\phi$ is conformal to~$G$ (keeps the left/right relation between every two non-intersecting chords),
the transitive orientations of $(S_i,{\parallel})$ induced by the permutation models $(\phi|S^0_i,\phi|S^1_i)$ are the same.
We denote this transitive orientation by ${<_{S_i}}$.
The triple $\SSS_i = (S^0_i,S^1_i,{<_{S_i}})$ is called the \emph{metachord} and 
the sets $S^0_i$ and $S^1_i$ are called the \emph{slots} of the CA-module $S_i$.
The set $\slots =\{S^0_1,S^1_1,\ldots,S^0_t,S^1_t\}$ of slots and the set $\metachords = \{ \SSS_1,\ldots,\SSS_t\}$ of metachords are the components of $\dataStructure$.
For the metachord $\SSS_i$ it is convenient to assume the following definition.
\begin{definition}
\label{def:admissible-models-for-metachord}
A permutation model $\tau = (\tau^0,\tau^1)$ of $(S_i,{\sim})$ is \emph{admissible by $\mathbb{S}_i$} if:
\begin{itemize}
 \item $\tau^j$ is a permutation of $S^j_i$ for $j \in \{0,1\}$,
 \item we have ${<_{\tau}} = {<_{S_i}}$ (${\prec_{\tau}}$ is not restricted), where ${<_{\tau}}$ and ${\prec_{\tau}}$ are transitive orientations 
 of $(S_i,{\parallel})$ and $(S_i,{\sim})$, respectively, corresponding to $\tau$.
\end{itemize}
\end{definition}
Then, Lemma~\ref{lem:CA-modules} allows us to treat any conformal model $\phi$ as a collection of 
$t$ permutation models $(\phi|S^0_1, \phi|S^1_1), \ldots, (\phi|S^0_t, \phi|S^1_t)$  admissible by the metachords $\SSS_1,\ldots,\SSS_t$ and spanned between the slots $S^0_1 \leftrightarrow S^1_1, \ldots, S^0_t \leftrightarrow S^1_t$, respectively.
See Figure~\ref{fig:example_metachords} to the left.

Let $\phi$ be a conformal model of~$G$.
Denote by $\pi(\phi)$ the \emph{circular order of the slots in $\phi$}, that is, the circular order of $\slots$ obtained from $\phi$ by substituting every contiguous subword $\phi|S^j_i$ by the letter $S^j_i$. 
Usually we draw $\pi(\phi)$ in the way shown 
in Figure~\ref{fig:example_metachords}, that is, for every two corresponding slots $S^0_i$ and $S^1_i$ placed on the circle we draw a chord oriented from $S^0_i$ to $S^1_i$.
Since such a chord represents a model admissible for the metachord $\SSS_i$, 
we call it simply the \emph{metachord} of $\SSS_i$.

\input ./figures/data_structure/example_metachords.tex

The last component~$\Pi$ of the data structure~$\dataStructure$ contains the set of \emph{circular orders of the slots} that might appear in the conformal models of~$G_{ov}$, that is,
$$\Pi = \{\pi(\phi): \phi \text{ is a conformal model of }G_{ov}\}.$$
In particular, we can generate any conformal model of~$G_{ov}$ by:  
\begin{itemize}
 \item picking a circular order of the slots $\pi$ from the set $\Pi$,
 \item replacing the slots $S^0_i$ and $S^1_i$ in $\pi$ by words~$\tau^0_i$ and~$\tau^1_i$, 
 where $(\tau^0_i,\tau^1_i)$ is an oriented permutation model of~$(S_i,{\sim})$ admissible by the metachord $\mathbb{S}_i$.
\end{itemize}

The set $\Pi$ might have exponentially many members, however, it has a linear-size representation by means of a \emph{PQS-tree} of $G$ -- see Subsection~\ref{sub:PQS_tree} for more details.

The rest of this section is organized as follows:
\begin{itemize}
 \item In Subsection~\ref{sub:PQS_tree} we describe the PQS-tree of~$G$ and we show 
 how it represents the set~$\Pi$. 
 We also show how to read the PQS-tree from a given conformal model of~$G_{ov}$.
 \item In Subsection~\ref{sub:admissible_models} we describe the structure of all admissible models for 
 a single metachord.
 \item In Subsection~\ref{sub:PQSM_tree} we introduce the PQSM-tree $\pqsmtree$ and we show how it represents the conformal models of~$G_{ov}$.
\end{itemize}

\subsection{PQS-tree}
\label{sub:PQS_tree}

In this subsection we show how to construct the PQS-tree $\pqstree$.
The PQS-tree~$\pqstree$ is an unrooted tree. 
Its leaf nodes, which are also called as \emph{S-nodes} of $\pqstree$, correspond to the slots of $G$. 
The \emph{Q-nodes} correspond to the connected components of $G_{ov}$.
An edge is added between a slot $S^j_i$ and a Q-node $Q$ if $S_i \subseteq Q$.
This finishes the construction of $\pqstree$ when $V$ is serial or prime. 
In these cases, $V$ is the only component of $G_{ov}$, and $\pqstree$ 
consists of a single inner Q-node $V$ and the slots from $\slots$ adjacent to $V$.

To complete the definition for the case where $V$ is parallel in $G_{ov}$ (then $G_{ov}$ has at least two components), an additional preparation is required. 
Let $Q_0$ and $Q_1$ be two components of $G_{ov}$.
We say $Q_0$ and $Q_1$ are \emph{separated} if there exists a vertex $v \in V \setminus (Q_0  \cup Q_1)$ such that $Q_i \subseteq \leftside(v)$ and $Q_{1-i} \subseteq \rightside(v)$ for some $i \in \{0,1\}$. 
Otherwise, $Q_0$ and $Q_1$ are \emph{neighboring}.
The inner nodes of the PQS-tree $\pqstree$ includes both Q-nodes, which correspond to the components of $G_{ov}$, and P-nodes. 
The \emph{P-nodes} correspond to the maximal sets of pairwise neighboring Q-nodes 
(note that $|P| \geq 2$ for any P-node $P$).
An edge is added between a Q-node $Q$ and a P-node $P$ if $Q \in P$.
This completes the definition of~$\pqstree$ for the case when $V$ is parallel.
See Figure~\ref{fig:PQS_tree} for an illustration.


\input ./figures/data_structure/pq-tree/pqtree.tex

We represent the set $\Pi$ through the sets $\Pi(N)$ of (possible) \emph{orderings} of a node $N$, 
which are defined for all inner nodes $N$ of the PQS-tree $\pqstree$.
For every inner node $N$ of $\pqstree$, the set $\Pi(N)$ contains some circular orders of the set of the neighbours of $N$ in~$\pqstree$ (the precise definition of~$\Pi(N)$ will be given later on).
The PQS-tree~$\pqstree$ is said to be \emph{ordered} if every inner node~$N$ in~$\pqstree$ is assigned 
an ordering from the set~$\Pi(N)$.
Every ordered PQS-tree~$\pqstree$ \emph{represents} a circular order of the set~$\slots$, as follows:
we embed $\pqstree$ in the plane in such a way the clockwise order of the neighbours of every inner node~$N$ is consistent with the assigned ordering from $\Pi(N)$ and then we list all the slots as they occur when we walk the boundary of~$\pqstree$ in the clockwise order.
The sets $\Pi(\cdot)$ will be defined such that there is the correspondence between the members of~$\Pi$ and the circular orders of $\slots$ represented by the ordered PQS-trees~$\pqstree$.
Hence, for $\pi \in \Pi$ we denote the ordered tree representing $\pi$ by~$\pqstree_{\pi}$ and,
for any inner node~$N$ in $\pqstree$, by $\pi_{|N}$ we denote the ordering (which is in the set $\Pi(N)$) of the node~$N$ in the ordered tree $\pqstree_{\pi}$.
In particular, for every inner node $N$ of $\pqstree$ we have
$$\Pi(N) = \{\pi_{|N}: \pi \in \Pi \}.$$

Next we show how to determine for a given $\pi \in \Pi$ the ordered tree $\pqstree_{\pi}$ representing $\pi$.
We can achieve this by defining $\pi_{|N}$ for every inner node in $\pqstree$.

Clearly, if $V$ is serial/prime, we set $\pi_{|V} = \pi$. 

Suppose $V$ is parallel.
Let $Q$ be a Q-node and $P$ be a P-node such that $Q$ and $P$ are adjacent in $\pqstree$.
When we delete the node $Q$ from $\pqstree$, we obtain a forest, 
and one of its components contains the node $P$.
Let $\slots_{\pqstree - Q}(P)$ denote the set of all slots in the component containinig $P$.
Similarily, when we delete the node $P$ from $\pqstree$, we obtain a forest, 
and one of its components contains the node $Q$.
Let $\slots_{\pqstree - P}(Q)$ denote the set of all slots in the component containinig $Q$.
In \cite{Kra24} the following property of every circular order of the slots~$\pi$ from $\Pi$ with respect to the nodes $Q$ and $P$ is shown:
\begin{itemize}
 \item the slots from the set $\slots_{\pqstree - Q}(P)$ form a contiguous subword in $\pi$,
 \item the slots from the set $\slots_{\pqstree - P}(Q)$ form a contiguous subword in $\pi$.
\end{itemize}
See Figure~\ref{fig:PQS_tree}. 
Now,
\begin{itemize}
\item for every Q-node $Q$ let $\pi_{|Q}$ be a circular word obtained from $\pi$ by substituting the contiguous subword $\slots_{\pqstree - Q}(P)$ by the letter $P$, for every P-node $P$ adjacent to $Q$.
Note that $\pi_{|Q}$ is the circular permutation of the neighbours of $Q$ in $\pqstree$.
\item for every P-node $P$ we obtain $\pi_{|P}$ from $\pi$ by substituting the contiguous subword $\slots_{\pqstree - P}(Q)$ by the letter $Q$, for every Q-node $Q$ adjacent to $P$.
Note that $\pi_{|P}$ is the circular permutation of the neighbours of $P$ in $\pqstree$.
\end{itemize}
We might easily check that, if we order each inner node $N$ of $\pqstree$ consistently with $\pi_{|N}$,
we obtain the ordered PQS-tree representing $\pi$.
See Figure~\ref{fig:PQS_tree}.


The definition of the sets $\Pi(\cdot)$ differs depending on whether~$V$ is serial/prime/parallel in~$\strongModules(G_{ov})$.
Again, in this section we show how to determine the sets $\Pi(\cdot)$ given the conformal model~$\phi$ of~$G_{ov}$.

\subsubsection{$V$ is serial in $\strongModules(G_{ov})$}
In this case we have $\camodules(M)=\{M\}$ for any child $M$ of $V$ in $\strongModules(G_{ov})$ -- see \cite{Kra24} for more details.
Hence the set of CA-modules $\camodules$ of $G$ coincides with the set of children of $V$ in $\strongModules(G_{ov})$.
Let $\camodules = \{S_1,\ldots,S_t\}$.
Then, \cite{Kra24} shows that 
$$
\Pi(V) =  \left \{ \pi :
\begin{array}{c}
\text{$\pi$ is a circular order of $S^0_1,S^1_1,\ldots,S^0_t,S^1_t$ such that for every } \\
\text{distinct $i,j \in [t]$ the slots associated with $S_i$ and $S_j$ overlap} 
\end{array}
\right \}.
$$
In particular, we have $\Pi = \Pi(V)$.
See Figure~\ref{fig:Pi-serial} for an illustration.

\begin{center}
\input ./figures/data_structure/pq-tree/serial/pi_serial_case.tex
\end{center}

\subsubsection{$V$ is prime in $\strongModules(G_{ov})$}
In this case, when $M$ is a prime child of $V$, we have $\camodules(M) = \{M\}$, 
and when $M$ is a serial/parallel child of $V$ every CA-module in $\camodules(M)$ is 
the union of some children of $M$ in $\strongModules(G_{ov})$.
Let $\camodules = \{S_1,\ldots,S_t\}$ and let $\pi = \pi(\phi)$.
Then, \cite{Kra24} proves that
$$\Pi(V) = \{\pi,\pi^R\},$$
where $\pi^R$ is the reflection of $\pi$. 
In particular, we have $\Pi = \Pi(V)$.
See Figure~\ref{fig:Pi-prime} for an illustration.
\begin{center}
\input ./figures/data_structure/pq-tree/prime/pi_prime_case.tex
\end{center}

\subsubsection{$V$ is parallel in $\strongModules(G_{ov})$}
In this case the children of $V$ in $\strongModules(G_{ov})$ correspond to the 
connected components of $G_{ov}$, which in turn correspond to the Q-nodes in the PQS-tree~$\pqstree$.
We recall that $\camodules(Q)$ forms a partition of $Q$, for every Q-node $Q$ of $\pqstree$.
Then, \cite{Kra24} proves that:
\begin{itemize}
 \item for a P-node $P$ the set $\Pi(P)$ contains all circular permutations of the neighbours of~$P$ in~$\pqstree$,
 \item for a Q-node $Q$ the set $\Pi(Q)$ contains two circular permutations of the neighbours of $Q$ in $\pqstree$, one being the reflection of the other. 
 In particular, given any $\pi \in \Pi$, the set $\Pi(Q)$ contains $\pi_{|Q}$ and its reflection $(\pi_{|Q})^R$.
\end{itemize}
We note that we might have $\pi_{|Q} \equiv (\pi_{|Q})^R$, which takes place if and only if $\camodules(Q)=\{Q\}$.
If the above holds, $Q$ is called a \emph{permutation} component.

Eventually, note that, given $\pi \in \Pi$ and $\pqstree_{\pi}$ representing $\pi$, 
any circular order of the slots in $\Pi$ can be obtained by performing a sequence of operations on the ordered PQS-tree~$\pqstree_{\pi}$, where each of them either
\begin{itemize}
 \item reflects a Q-node, or
 \item permutes arbitrarily the neighbours of a P-node.
\end{itemize}
The \emph{reflection of a Q-node} $Q$ transforms $\pqstree_\pi$ into $\pqstree_{\pi'}$, 
where the only difference between $\pqstree_{\pi}$ and $\pqstree_{\pi'}$ is an ordering of the node $Q$:
$\pqstree_{\pi}$ orders the neighbours of $Q$ according to $\pi_{|Q}$ while
$\pqstree_{\pi'}$ orders the neighbours of $Q$ according to $(\pi_{|Q})^R$.
See Figure~\ref{fig:Q-node-reflection} for an illustration.
\input ./figures/data_structure/pq-tree/parallel/Q_node_reflection.tex

A \emph{permutation of a P-node} $P$ transforms $\pqstree_\pi$ into $\pqstree_{\pi'}$, 
where the only difference between $\pqstree_{\pi}$ and $\pqstree_{\pi'}$ is an ordering of the node $P$:
$\pqstree_{\pi}$ orders the neighbours of $Q$ consistently with $\pi_{|P}$ and 
$\pqstree_{\pi'}$ orders the neighbours of $Q$ consistently with $\pi'_{|P}$, where $\pi'_{|P}$ is any circular order of the neighbours of $P$.
See Figure~\ref{fig:P-node-permutation} for an illustration.
\input{./figures/data_structure/pq-tree/parallel/P_node_permutation.tex}



\subsection{The structure of the admissible models of a metachord}
\label{sub:admissible_models}
Let $S$ be a CA-module of $G$ and let 
$\SSS = (S^0,S^1,{<_{S}})$ be the metachord associated with~$S$.
Clearly, the subgraph of $G$ induced by the set $S$ is co-bipartite, 
and hence we can describe the structure of the admissible models for $\SSS$
basing on the work of Spinrad~\cite{Spin88} described in Section~\ref{sec:related_work}.
We recall that, due to Theorem~\ref{thm:permutation_models_transitive_orientations}, the models admissible by $\mathbb{S}$ are in the correspondence with the transitive orientations of the permutation graph $(S,{\sim})$.

First, note that for any admissible model $\tau = (\tau^0,\tau^1)$ for $\SSS$
its reflection $\mu = (\mu^0,\mu^1)$ is also admissible by $\SSS$.
Note that: 
\begin{itemize}
 \item if $\tau$ and $\mu$ correspond to the transitive orientations 
${\prec_{\tau}}$ and ${\prec_{\mu}}$ of $(S,{\sim})$, then $\prec_{\mu}$ is the reverse of $\prec_{\tau}$,
 \item $\mu^0$ is the reflection of~$\tau^1$ and $\mu^1$ is the reflection of~$\tau^0$.
\end{itemize}
See Figure~\ref{fig:admissible-model-reflection} for an illustration.

\input ./figures/data_structure/admissible_models/admissible_model_reflection.tex

From now we call the modules in $\strongModules(S,{\sim})$ as \emph{nodes} of the tree $\strongModules(S,{\sim})$  
and the inner nodes in $\strongModules(S,{\sim})$ as \emph{M-nodes} of the tree in $\strongModules(S,{\sim})$.
Since $(S,{<_S})$ might have a quadratic size, we need to find a way to represent the admissible way of $\SSS$ in linear space.
First, for a node $M \in \strongModules(S,{\sim})$ we define the \emph{metachord $\MMM$} of $M$ as the triple $(M^0,M^1,{<_M})$, where $M^0 = M^* \cap S^0$, $M^1 = M^* \cap S^1$, and ${<_M}$ equals to ${<_{S}}$ restricted to $M$.
Recall that for every admissible model $(\tau^0,\tau^1)$ for $\SSS$ and for every $j \in \{0,1\}$ 
the set $M^j$ is contiguous in $\tau^j$, and for any child $K$ of $M$ in~$\strongModules(S,{\sim})$ the set $K^j$ is contiguous in the word~$\tau^j|M^j$.
Then, for every M-node~$M$ we define the set $\Pi(M)$ of possible \emph{orderings} of the children of 
$M$ in the words $\tau^0|M^0$ and $\tau^1|M^1$, that is, each member~$(\pi^0,\pi^1)$ of~$\Pi(M)$ 
determines the order in which the contiguous sets $K^0$ and $K^1$ associated with the children $K$ of $M$ 
may occur in the words $\tau^0|M^0$ and $\tau^1|M^1$, respectively.
Formally, for every transitive orientation ${\prec_M}$ of $(M,{\sim}_M)$ we have an ordering $\pi_M=(\pi^0, \pi^1)$ in the set $\Pi(M)$, where the word $\pi^j$ for $j \in \{0,1\}$ is a permutation of the set $\{K^j: K \text{ is a child of $M$ in } \strongModules(S,{\sim})\}$ such that for every two distinct children $K,L$ of $M$:
\begin{equation}
\begin{array}{lll}
K^0 \text{ occurs before } L^0 \text{ in } \pi^{0} \iff K \prec_M L \text{ or } K <_{M} L,\\
K^1 \text{ occurs before } L^1 \text{ in } \pi^{1} \iff K \prec_M L \text{ or } L <_{M} K.\\
\end{array}
\end{equation}
Figure~\ref{fig:admissible-model-structure} shows a modular decomposition tree $\strongModules(S,{\sim})$ for some CA-module $S$ and its admissible model $\tau = (\tau^0,\tau^1)$.
The M-node $S$ is prime, $(S,{\sim_S})$ has two transitive orientations, one being the reverse of the other,
and the set $\Pi(S)$ has two orderings: $(A^0_1A^0_2A^0_3A^0_4, A^1_2A^1_4A^1_1A^1_3)$ and its reflection $(A^0_3A^0_1A^0_4A^0_2, A^1_4A^1_3A^1_2A^1_1)$.
The M-node $A_2$ is serial with three children, $(A_2,{\sim_{A_2}})$ 
has $3!$ transitive orientations corresponding to the linear orders of its children $B_1,B_2,B_3$, 
and the set $\Pi(A_2)$ has $3!$ orderings $(B^0_iB^0_jB^0_k, B^1_iB^1_jB^1_k)$ corresponding to all permutations $i,j,k$ of the set $[3]$.
The remaining M-nodes $A_3, B_2, B_3$ are parallel, each graph $(A_3,{\sim_{A_3}})$, $(B_2,{\sim_{B_2}})$, $(B_3,{\sim_{B_3}})$ has one (empty) transitive orientation, and each set $\Pi(A_3)$, $\Pi(B_2)$, and $\Pi(B_3)$
has one possible ordering.
For example, we have $\Pi(A_3) = \big{\{} (B^0_4 B^0_5, B^1_5 B^1_4) \big{\}}$.

For any $M$-node $M$ we can represent the set $\Pi(M)$ in space linear in the number of children of $M$ in $\strongModules(S,{\sim})$
(for a serial M-node $M$ it suffices to represent the type of $M$ and one member of $\Pi(M)$).
Hence, we can represents all the sets $\Pi(M)$ for all $M$-nodes in space linear in the size of $\strongModules(S,{\sim})$, and hence linear in the size of $(S,{\sim})$.




Following our convention, tree $\strongModules(S,{\sim})$ is said to be \emph{ordered} if every M-node in $\strongModules(S,{\sim})$ is assigned an ordering from the set~$\Pi(M)$.
Theorems~\ref{thm:transitive_orientations_versus_transitive_orientations_of_strong_modules} and~\ref{thm:permutation_models_transitive_orientations} assert one-to-one correspondence between admissible models~$\tau$ for~$\SSS$ and the ordered trees~$\strongModules(S,{\sim})$.
For every admissible model $\tau$ for $\SSS$, by $\tau_{|M}$ we denote the ordering of the node $M$ in the ordered tree $\strongModules(S,{\sim})_{\tau}$ corresponding to $\tau$ -- see Figure~\ref{fig:admissible-model-structure} for an illustration. 


\input ./figures/data_structure/admissible_models/admissible_model_structure.tex


\subsection{PQSM-tree of $G$}
\label{sub:PQSM_tree}
We obtain the \emph{PQSM-tree} $\pqsmtree$ of $G$ by attaching the root $S$ of the modular decomposition tree $\strongModules(S,{\sim})$ to the leaf slot $S^0$ of the PQS-tree $\pqstree$ of $G$, for every $S \in \mathcal{S}$.
A node $N$ of $\pqsmtree$ is a \emph{PQM-node} in if $N$ is either a P-node, or a Q-node, or an M-node.
Note that the set~$\Pi(N)$ is defined for all PQM-nodes in~$\pqsmtree$.
Following our convention, we say PQSM-tree~$\pqsmtree$ is \emph{ordered} if every PQM-node~$N$ in~$\pqsmtree$ is assigned an ordering in the set~$\Pi(N)$.
Clearly, there is one-to-one correspondence between the ordered PQSM-trees
and the conformal models of~$G_{ov}$.
For a conformal model~$\phi$ of~$G_{ov}$ and a PQM-node~$N$ in~$\pqsmtree$ 
by~$\phi_{|N}$ we denote the ordering of the node~$N$ in the ordered PQSM-tree~$\pqsmtree_{\phi}$ corresponding to $\phi$.



==> figures/intro/Spinrad_relation.tex <==
\begin{figure}[htp!]
%uv_disjoint\begin{tikzpicture}[scale=1,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\begin{tikzpicture}[scale=0.9,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (label) at (0,-3) {};

\coordinate (A) at (-1,0) {};
\coordinate (B) at (1,0) {};
\coordinate (lA) at (-1.3,0) {};
\coordinate (lB) at (1.3,0) {};

\coordinate (lu) at (-0.7,0.7) {};
\coordinate (lv) at (0.3,1.2) {};
%\coordinate (lu1) at (-0.25,1.25) {};
%\coordinate (lv1) at (1.25,0) {};

%v
\draw[red,thick, rounded corners] (0.5, -1) -- (-1,-1) -- (-1,1)--(0.5,1);
\draw[red, dashed] (0.5, -1) -- (0.5,1);
%u
\draw[thick, rounded corners] (-0.5, -0.9) -- (-0.9,-0.9) -- (-0.9,0.9)--(-0.5,0.9);
\draw[dashed] (-0.5, -0.9) -- (-0.5,0.9);

\draw[] (-1.1, 0) -- (-0.8,0);
\draw[] (0.9, 0) -- (1.1,0);


\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lA) {$A$};
\node at (lB) {$B$};
\node at (lu) {$u$};
\node at (lv) {$v$};
\end{scriptsize}


\draw[white] (-1.5,-1.5)--(-1.5,1.5);
\draw[white] (1.5,-1.5)--(1.5,1.5);
\end{tikzpicture}
\hspace{0.4cm}
\begin{tikzpicture}[scale=0.9,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (label) at (0,-3) {};

\coordinate (A) at (-1,0) {};
\coordinate (B) at (1,0) {};
\coordinate (lA) at (-1.3,0) {};
\coordinate (lB) at (1.3,0) {};

\coordinate (lu) at (-0.3,0.7) {};
\coordinate (lv) at (0.7,0.7) {};
%\coordinate (lu1) at (-0.25,1.25) {};
%\coordinate (lv1) at (1.25,0) {};

%v
\draw[red,thick, rounded corners] (0.5, -0.9) -- (0.9,-0.9) -- (0.9,0.9)--(0.5,0.9);
\draw[red, dashed] (0.5, -0.9) -- (0.5,0.9);
%u
\draw[thick, rounded corners] (-0.5, -1) -- (1,-1) -- (1,1)--(-0.5,1);
\draw[dashed] (-0.5, -1) -- (-0.5,1);

\draw[] (-1.1, 0) -- (-0.9,0);
\draw[] (0.8, 0) -- (1.1,0);


\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lA) {$A$};
\node at (lB) {$B$};
\node at (lu) {$u$};
\node at (lv) {$v$};
\end{scriptsize}


\draw[white] (-1.5,-1.5)--(-1.5,1.5);
\draw[white] (1.5,-1.5)--(1.5,1.5);
\end{tikzpicture}
\hspace{0.4cm}
\begin{tikzpicture}[scale=0.9,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (label) at (0,-3) {};

\coordinate (A) at (-1,0) {};
\coordinate (B) at (1,0) {};
\coordinate (lA) at (-1.3,0) {};
\coordinate (lB) at (1.3,0) {};

\coordinate (lu) at (-0.7,1.2) {};
\coordinate (lv) at (0.7,1.2) {};
%\coordinate (lu1) at (-0.25,1.25) {};
%\coordinate (lv1) at (1.25,0) {};

%v
\draw[red,thick, rounded corners] (0.5, 1) -- (1,1) -- (1,-1)--(0.5,-1);
\draw[red, dashed] (0.5, -1) -- (0.5,1);
%u
\draw[thick, rounded corners] (-0.5, -1) -- (-1,-1) -- (-1,1)--(-0.5,1);
\draw[dashed] (-0.5, -0.9) -- (-0.5,0.9);

\draw[] (-1.1, 0) -- (-0.9,0);
\draw[] (0.9, 0) -- (1.1,0);


\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lA) {$A$};
\node at (lB) {$B$};
\node at (lu) {$u$};
\node at (lv) {$v$};
\end{scriptsize}


\draw[white] (-1.5,-1.5)--(-1.5,1.5);
\draw[white] (1.5,-1.5)--(1.5,1.5);
\end{tikzpicture}
\hspace{0.4cm}
\begin{tikzpicture}[scale=0.9,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (label) at (0,-3) {};

\coordinate (A) at (-1,0) {};
\coordinate (B) at (1,0) {};
\coordinate (lA) at (-1.3,0) {};
\coordinate (lB) at (1.3,0) {};

\coordinate (lu) at (-0.3,0.7) {};
\coordinate (lv) at (0.3,1.2) {};
%\coordinate (lu1) at (-0.25,1.25) {};
%\coordinate (lv1) at (1.25,0) {};

%v
\draw[red,thick, rounded corners] (0.5, -1) -- (-1,-1) -- (-1,1)--(0.5,1);
\draw[red,dashed] (0.5, -1)--(0.5,1);
%u
\draw[thick, rounded corners] (-0.5, -0.9) -- (1,-0.9) -- (1,0.9)--(-0.5,0.9);
\draw[dashed] (-0.5, -0.9) -- (-0.5,0.9);

\draw[] (-1.1, 0) -- (-0.9,0);
\draw[] (0.9, 0) -- (1.1,0);


\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lA) {$A$};
\node at (lB) {$B$};
\node at (lu) {$u$};
\node at (lv) {$v$};
\end{scriptsize}


\draw[white] (-1.5,-1.5)--(-1.5,1.5);
\draw[white] (1.5,-1.5)--(1.5,1.5);
\end{tikzpicture}
\caption{\label{fig:Spinrad_relation} Spinrad sets $u < v$ if and only if either $u,v \in C_A$ and $u$ is contained in $b$ (left) or $u,v \in C_B$ and $u$ contains $b$ (middle left) or $u \in C_A$, $v \in C_B$, and $u,v$ are disjoint, or $u \in C_B$, $v \in C_A$, and $u,v$ cover the circle.}
\end{figure}


==> figures/intro/arc_placements.tex <==
\begin{figure}[htp!]
%disjoint
\begin{tikzpicture}[scale=0.5]
\coordinate (center) at (0,0) {};
\coordinate (v) at ($(center)+(90:2cm)$) {};
\coordinate (u) at ($(center)+(270:2cm)$) {};

\coordinate (lv) at ($(center)+(90:2.6cm)$) {};
\coordinate (lu) at ($(center)+(270:2.6cm)$) {};

\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lv) {$\psi(v)$};
\node at (lu) {$\psi(u)$};
\end{scriptsize}

%u
\draw[thick] ([shift=(30:2.1cm)]0,0) arc (30:150:2.1cm);
%u
\draw[thick] ([shift=(210:2.1cm)]0,0) arc (210:330:2.1cm);

\draw[thick, white] (-3.0,-3)--(-3.0,-2.8);
\draw[thick, white] (3.0,3)--(3.0,2.8);

\end{tikzpicture}
%contains
\begin{tikzpicture}[scale=0.5]
\coordinate (center) at (0,0) {};
\coordinate (v) at ($(center)+(90:2cm)$) {};
\coordinate (u) at ($(center)+(270:2cm)$) {};

\coordinate (lv) at ($(center)+(90:2.6cm)$) {};
\coordinate (lu) at ($(center)+(90:1.25cm)$) {};

\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lv) {$\psi(v)$};
\node at (lu) {$\psi(u)$};
\end{scriptsize}

%v
\draw[thick] ([shift=(0:2.1cm)]0,0) arc (0:180:2.1cm);
%u
\draw[thick] ([shift=(45:1.8cm)]0,0) arc (45:135:1.8cm);

\draw[thick, white] (-3.0,-3)--(-3.0,-2.8);
\draw[thick, white] (3.0,3)--(3.0,2.8);

\end{tikzpicture}
%is_contained
\begin{tikzpicture}[scale=0.5]
\coordinate (center) at (0,0) {};
\coordinate (v) at ($(center)+(90:2cm)$) {};
\coordinate (u) at ($(center)+(270:2cm)$) {};

\coordinate (lu) at ($(center)+(90:2.6cm)$) {};
\coordinate (lv) at ($(center)+(90:1.25cm)$) {};

\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lv) {$\psi(v)$};
\node at (lu) {$\psi(u)$};
\end{scriptsize}

%v
\draw[thick] ([shift=(0:2.1cm)]0,0) arc (0:180:2.1cm);
%u
\draw[thick] ([shift=(45:1.8cm)]0,0) arc (45:135:1.8cm);

\draw[thick, white] (-3.0,-3)--(-3.0,-2.8);
\draw[thick, white] (3.0,3)--(3.0,2.8);

\end{tikzpicture}
%cover_the_circle
\begin{tikzpicture}[scale=0.5]
\coordinate (center) at (0,0) {};
\coordinate (v) at ($(center)+(90:2cm)$) {};
\coordinate (u) at ($(center)+(270:2cm)$) {};

\coordinate (lv) at ($(center)+(90:2.6cm)$) {};
\coordinate (lu) at ($(center)+(270:2.4cm)$) {};

\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lv) {$\psi(v)$};
\node at (lu) {$\psi(u)$};
\end{scriptsize}

%v
\draw[thick] ([shift=(-20:2.1cm)]0,0) arc (-20:200:2.1cm);
%u
\draw[thick] ([shift=(160:1.9cm)]0,0) arc (160:380:1.9cm);

\draw[thick, white] (-3.0,-3)--(-3.0,-2.8);
\draw[thick, white] (3.0,3)--(3.0,2.8);

\end{tikzpicture}
%overlap
\begin{tikzpicture}[scale=0.5]
\coordinate (center) at (0,0) {};
\coordinate (v) at ($(center)+(90:2cm)$) {};
\coordinate (u) at ($(center)+(270:2cm)$) {};

\coordinate (lv) at ($(center)+(90:2.6cm)$) {};
\coordinate (lu) at ($(center)+(270:2.4cm)$) {};

\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lv) {$\psi(v)$};
\node at (lu) {$\psi(u)$};
\end{scriptsize}
\draw[thick] ([shift=(70:2.1cm)]0,0) arc (70:200:2.1cm);
\draw[thick] ([shift=(160:1.9cm)]0,0) arc (160:290:1.9cm);

\draw[thick, white] (-3.0,-3)--(-3.0,-2.8);
\draw[thick, white] (3.0,3)--(3.0,2.8);
\end{tikzpicture}

\caption{\label{fig:mutual_arc_position} From left to right:
$\psi(v)$ and $\psi(u)$ are disjoint, $\psi(v)$ contains $\psi(u)$, $\psi(v)$ is contained in $\psi(u)$,
$\psi(v)$ and $\psi(u)$ cover the circle, and $\psi(v)$ and $\psi(u)$ overlap.
}

\end{figure}


==> figures/intro/straightening_bending.tex <==
\begin{figure}[htp!]
\begin{tikzpicture}[xscale=0.80,yscale=0.80,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]

\coordinate (lphiv) at (1.5,0) {};
\coordinate (lpsiv) at (-1.5,0) {};

\coordinate (lpsiv) at ($(center)+(160:1.5cm)$) {};
\coordinate (lphiv) at ($(center)+(160:-0.15cm)$) {};


\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lphiv) {$\phi(v)$};
\node at (lpsiv) {$\psi(v)$};
\end{scriptsize}

\draw (0,0) circle (2cm);
\draw[very thick] ([shift=(80:2cm)]0,0) arc (80:240:2cm);
\draw[red,<-,very thick] ([shift=(80:2cm)]0,0)--([shift=(240:2cm)]0,0);
\end{tikzpicture} 
\caption{\label{fig:straightening_bending} The transformation of the arc~$\psi(v)$ into the oriented chord~$\phi(v)$.}
\end{figure}


==> figures/intro/uv_pairs.tex <==
\begin{figure}[htp!]
%uv_disjoint
\begin{tikzpicture}[scale=0.6,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (label) at (0,-3) {};

\coordinate (lv) at (-0.3,0) {};
\coordinate (lu) at (1.35,0) {};

\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lv) {$v$};
\node at (lu) {$u$};
\end{scriptsize}

%u
\draw[thick] ([shift=(-60:2.2cm)]0,0) arc (-60:60:2.2cm);
\draw[thick,<-] ([shift=(-60:2.2cm)]0,0) -- ([shift=(60:2.2cm)]0,0);

%v
\draw[red, thick] ([shift=(90:2.0cm)]0,0) arc (90:270:2.0cm);
\draw[red, thick,<-] ([shift=(90:2.0cm)]0,0) -- ([shift=(270:2.0cm)]0,0);

%\draw[thick,red] ([shift=(80:3cm)]0,0) arc (80:130:3cm);
\draw[white] (-2.5,-2.5)--(-2.5,-2.3);
\draw[white] (2.5,2.5)--(2.5,2.3);
\end{tikzpicture}
\hspace{0.2cm}
%v_contains_u
\begin{tikzpicture}[scale=0.6,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (label) at (0,-3) {};

\coordinate (lv) at (0.3,0) {};
\coordinate (lu) at (-1.25,0) {};

\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lv) {$v$};
\node at (lu) {$u$};
\end{scriptsize}

%u
\draw[thick] ([shift=(120:2.0cm)]0,0) arc (120:240:2.0cm);
\draw[thick,->] ([shift=(240:2.0cm)]0,0) -- ([shift=(120:2.0cm)]0,0);

%v
\draw[red, thick] ([shift=(90:2.2cm)]0,0) arc (90:270:2.2cm);
\draw[red, thick,<-] ([shift=(90:2.2cm)]0,0) -- ([shift=(270:2.2cm)]0,0);

%\draw[thick,red] ([shift=(80:3cm)]0,0) arc (80:130:3cm);
\draw[white] (-2.5,-2.5)--(-2.5,-2.3);
\draw[white] (1.1,2.5)--(1.1,2.3);
\end{tikzpicture}
\hspace{0.2cm}
%v_is_contained_in_u
\begin{tikzpicture}[scale=0.6,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (label) at (0,-3) {};

\coordinate (lv) at (-0.3,0) {};
\coordinate (lu) at (1.35,0) {};

\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lv) {$v$};
\node at (lu) {$u$};
\end{scriptsize}

%u
\draw[thick] ([shift=(60:2.2cm)]0,0) arc (60:300:2.2cm);
\draw[thick,->] ([shift=(300:2.2cm)]0,0) -- ([shift=(60:2.2cm)]0,0);

%v
\draw[red, thick] ([shift=(90:2.0cm)]0,0) arc (90:270:2.0cm);
\draw[red, thick,<-] ([shift=(90:2.0cm)]0,0) -- ([shift=(270:2.0cm)]0,0);

%\draw[thick,red] ([shift=(80:3cm)]0,0) arc (80:130:3cm);
\draw[white] (-2.5,-2.5)--(-2.5,-2.3);
\draw[white] (2.3,2.5)--(2.3,2.3);
\end{tikzpicture}
\hspace{0.2cm}
%uv_cover_the_circle
\begin{tikzpicture}[scale=0.6,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (label) at (0,-3) {};

\coordinate (lv) at (0.3,0) {};
\coordinate (lu) at (-1.0,0) {};

\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lv) {$v$};
\node at (lu) {$u$};
\end{scriptsize}

%u
\draw[thick] ([shift=(250:2.0cm)]0,0) arc (250:470:2.0cm);
\draw[thick,<-] ([shift=(250:2.0cm)]0,0) -- ([shift=(470:2.0cm)]0,0);

%v
\draw[red, thick] ([shift=(90:2.2cm)]0,0) arc (90:270:2.2cm);
\draw[red, thick,<-] ([shift=(90:2.2cm)]0,0) -- ([shift=(270:2.2cm)]0,0);

%\draw[thick,red] ([shift=(80:3cm)]0,0) arc (80:130:3cm);
\draw[white] (-2.5,-2.5)--(-2.5,-2.3);
\draw[white] (2.5,2.5)--(2.5,2.3);
\end{tikzpicture}
\hspace{0.2cm}
%uv_overlap
\begin{tikzpicture}[scale=0.6,>=latex,shorten >=-0.4pt,shorten <=-0.4pt]
\coordinate (label) at (0,-3) {};

\coordinate (lv) at (-0.3,0) {};
\coordinate (lu) at (1.05,0.7) {};

\tikzstyle{every node}=[inner sep=1pt]
\begin{scriptsize}
\node at (lv) {$v$};
\node at (lu) {$u$};
\end{scriptsize}

%u
\draw[thick] ([shift=(30:2.0cm)]0,0) arc (30:150:2.0cm);
\draw[thick,<-] ([shift=(30:2.0cm)]0,0) -- ([shift=(150:2.0cm)]0,0);

%v
\draw[red, thick] ([shift=(90:2.2cm)]0,0) arc (90:270:2.2cm);
\draw[red, thick,<-] ([shift=(90:2.2cm)]0,0) -- ([shift=(270:2.2cm)]0,0);

%\draw[thick,red] ([shift=(80:3cm)]0,0) arc (80:130:3cm);
\draw[white] (-2.5,-2.5)--(-2.5,-2.3);
\draw[white] (2.5,2.5)--(2.5,2.3);
\end{tikzpicture}
\caption{\label{fig:uv_pairs} The possible relations between the arcs $\psi(v)$ and $\psi(u)$ and the corresponding oriented chords $\phi(v)$ and $\phi(u)$: $v$ is disjoint with $u$, $v$~contains~$u$, $v$~is contained in~$u$, $v$~and $u$~cover the circle, and $v$~and $u$~overlap, respectively.}
\end{figure}

